Measurements of the diffuse Galactic synchrotron spectral index and curvature from MeerKLASS pilot data

21cm intensity mapping experiments are bringing an influx of high spectral resolution observational data in the $\sim100$ MHz $- 1$ GHz regime. We use pilot $971-1075$ MHz data from MeerKAT in single-dish mode, recently used to test the calibration and data reduction scheme of the upcoming MeerKLASS survey, to probe the spectral index of diffuse synchrotron emission below 1 GHz within $145^{\circ} < \alpha < 180^{\circ}$, $-1^{\circ} < \delta < 8^{\circ}$. Through comparisons with data from the OVRO Long Wavelength Array and the Maipu and MU surveys, we find an average spectral index of $-2.75 < \beta < -2.71$ between 45 and 1055 MHz. By fitting for spectral curvature with a spectral index of the form $\beta + c \, {\rm{ln}}(\nu / 73~{\rm MHz})$, we measure $\beta = -2.55 \pm 0.13$ and $c = -0.12 \pm 0.05$ within our target field. Our results are in good agreement (within $1\sigma$) with existing measurements from experiments such as ARCADE2 and EDGES. These results show the calibration accuracy of current data and demonstrate that MeerKLASS will also be capable of achieving a secondary science goal of probing the interstellar medium.

==> journaldefs.tex <==
% bibliography and bibfile journal definitions (taken from aa.cls)

\def\aj{AJ}					% Astronomical Journal
\def\araa{ARA\&A}				% Annual Review of Astron and Astrophys
\def\apj{ApJ}					% Astrophysical Journal
\def\apjl{ApJL}					% Astrophysical Journal, Letters
\def\apjs{ApJS}					% Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}				% Applied Optics
\def\apss{Ap\&SS}				% Astrophysics and Space Science
\def\aap{A\&A}					% Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}				% Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}				% Astronomy and Astrophysics, Supplement
\def\azh{AZh}					% Astronomicheskii Zhurnal
\def\baas{BAAS}					% Bulletin of the AAS
\def\jrasc{JRASC}				% Journal of the RAS of Canada
\def\memras{MmRAS}				% Memoirs of the RAS
\def\mnras{MNRAS}				% Monthly Notices of the RAS
\def\pra{Phys.~Rev.~A}				% Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}				% Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}				% Physical Review C
\def\prd{Phys.~Rev.~D}				% Physical Review D
\def\pre{Phys.~Rev.~E}				% Physical Review E
\def\prl{Phys.~Rev.~Lett.}			% Physical Review Letters
\def\pasp{PASP}					% Publications of the ASP
\def\pasj{PASJ}					% Publications of the ASJ
\def\qjras{QJRAS}				% Quarterly Journal of the RAS
\def\skytel{S\&T}				% Sky and Telescope
\def\solphys{Sol.~Phys.}			% Solar Physics
\def\sovast{Soviet~Ast.}			% Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}			% Space Science Reviews
\def\zap{ZAp}					% Zeitschrift fuer Astrophysik
\def\nat{Nature}				% Nature
\def\iaucirc{IAU~Circ.}				% IAU Cirulars
\def\aplett{Astrophys.~Lett.}			% Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}		% Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}	% Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}			% Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}		% Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}			% Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}			% Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}			% Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}	% Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}		% Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}			% Nuclear Physics A
\def\physrep{Phys.~Rep.}			% Physics Reports
\def\physscr{Phys.~Scr}				% Physica Scripta
\def\planss{Planet.~Space~Sci.}			% Planetary Space Science
\def\procspie{Proc.~SPIE}			% Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

% end of file


